Learning to Sparsify Travelling Salesman Problem Instances

In order to deal with the high development time of exact and approximation algorithms for NP-hard combinatorial optimisation problems and the high running time of exact solvers, deep learning techniques have been used in recent years as an end-to-end approach to find solutions. However, there are issues of representation, generalisation, complex architectures, interpretability of models for mathematical analysis etc. using deep learning techniques. As a compromise, machine learning can be used to improve the run time performance of exact algorithms in a matheuristics framework. In this paper, we use a pruning heuristic leveraging machine learning as a pre-processing step followed by an exact Integer Programming approach. We apply this approach to sparsify instances of the classical travelling salesman problem. Our approach learns which edges in the underlying graph are unlikely to belong to an optimal solution and removes them, thus sparsifying the graph and significantly reducing the number of decision variables. We use carefully selected features derived from linear programming relaxation, cutting planes exploration, minimum-weight spanning tree heuristics and various other local and statistical analysis of the graph. Our learning approach requires very little training data and is amenable to mathematical analysis. We demonstrate that our approach can reliably prune a large fraction of the variables in TSP instances from TSPLIB/MATILDA (>85%$) while preserving most of the optimal tour edges. Our approach can successfully prune problem instances even if they lie outside the training distribution, resulting in small optimality gaps between the pruned and original problems in most cases. Using our learning technique, we discover novel heuristics for sparsifying TSP instances, that may be of independent interest for variants of the vehicle routing problem.

==> appendices.tex <==
\begin{subappendices}
\renewcommand{\thesection}{\Alph{section}}%
\section{MWST Extraction}
\label{sec:mwstextraction}

The extraction of the minimum-weight spanning trees in succession necessitates the removal from consideration those that have been already identified in a minimum spanning tree. Each time these edges are removed, a unique minimum spanning tree can be determined in the resultant pruned graph (see Figure \ref{fig:mwst}).

\begin{figure}[htp]
    \centering
    \includegraphics[width=0.9\textwidth]{mwst.png}
    \caption{Extracting MWST edges for $k=2$ iterations. (a): The complete graph underlying the routing problem \footnote{In order to make the images easier to parse, many of the edges of the actual complete graph are not visualised}. (b): A new graph $H$ is initialised, that contains all of the vertices of $G$, but none of the edges. (c): The MWST $T$ of $G$ is computed. (d): The edges $E'$ are removed from $G$ and added to $H$. (e): A new MWST, $T'$, is computed from the modified graph $G$. (f): The edges $E''$ of the new tree $T$ are added to the graph $H$ and removed from $G$. We can also consider $H$ to be a sparsification of $G$.}
    \label{fig:mwst}
\end{figure}

\section{Doubletree Insertion}
\label{sec:dbtinsertion}

The doubletree approximation for a metric TSP constructs an approximate tour by computing a MWST in the underlying graph, duplicating the tree edges, visiting them in pre-order depth-first search and then removing the shortcuts from the pre-order list from left to right. In this work we compute a doubletour approximation in exactly this manner, but also construct another doubletour, creating shortcuts from right to left in the pre-order list. This gives two approximate tours, each guaranteed to have $\tilde{\ell} \leq 2$, with many overlapping edges. In practice this leads to slightly higher sacrifice in the pruning rate than a single tour does alone. Each time in this work it is stated that doubletour approximations are inserted into the pruned graph, it is actually these two doubletours, which increase slightly the chance for a pruned graph to admit better optimal solutions.

\end{subappendices}

==> name.tex <==
\begin{figure}[htp]
    \centering
    \includegraphics[width=0.4\textwidth]{vrp_edges.png}
    \caption{Illustration of a solution to a basic vehicle routing problem. Three vehicles traverse the graph such that each vehicle leaves the depot, visits a disjoint set of customer vertices and finally returns to the depot node. These tours must respect the capacity constraints, that is they must have enough capacity $C$ to satisfy the demands of their customer sets. The decision problem here is one of determining which edges in the graph must be chosen to form the tours.}
    \label{fig:mwst}
\end{figure}
